Application of higher-order structural theory to bending and free vibration analysis of sandwich plates with CNT reinforced composite facesheets

In this paper, the bending and free flexural vibration behaviour of sandwich plates with carbon nanotube (CNT) reinforced facesheets are investigated using QUAD-8 shear flexible element developed based on higher-order structural theory. This theory accounts for the realistic variation of the displacements through the thickness, and the possible discontinuity in slope at the interface, and the thickness stretch affecting the transverse deflection. The in-plane and rotary inertia terms are considered in the formulation. The governing equations obtained using Lagrange's equation of motions are solved for static and dynamic analyses considering a sandwich plate with homogeneous core and CNT reinforced face sheets. The accuracy of the present formulation is tested considering the problems for which solutions are available. A detailed numerical study is carried out based on various higher-order models deduced from the present theory to examine the influence of the volume fraction of the CNT, core-to-face sheet thickness and the plate thickness ratio on the global/local response of different sandwich plates.

==> highOrder_mech.tex <==
The static analysis is conducted for carbon nanotube reinforced functionally graded sandwich plate with homogeneous core. The following two types of mechanical loading are considered:

\begin{itemize}
\item Sinusoidal loading: $q(x,y) = q_o \sin (\pi x/a) \sin (\pi y/b)$,
\item Uniformly distributed loading: $q(x,y) = q_o$.
\end{itemize}

where $q_o$ is the amplitude of the mechanical load. The physical quantities are nondimensionalized by relations, unless stated otherwise:
\begin{eqnarray}
\renewcommand{\arraystretch}{2}
(\overline{u},\overline{v}) = \frac{100E_o}{q_o h S^3}(u,v) \nonumber \\
\overline{w} = \frac{100E_o}{q_o h S^4}(w) \nonumber \\
(\overline{\sigma}_{xx},\overline{\sigma}_{yy},\overline{\sigma}_{xy}) = \frac{(\sigma_{xx},\sigma_{yy},\sigma_{xy})}{q_oS^2} \nonumber \\
(\overline{\sigma}_{xz},\overline{\sigma}_{yz}) = \frac{(\sigma_{xz},\sigma_{yz})}{q_oS}
\end{eqnarray}
where the reference value is taken as $E_o =$ 1 GPa and $S = a/h$. 

\paragraph{Validation} Before proceeding to the detailed analysis of the static response of the sandwich plate for the applied mechanical load, the present formulation is validated against available solutions in the literature.  In this case, only one layer is considered and the effect of type of CNT volume fraction distribution is also considered. PmPV~\cite{zhulei2012} is considered as the matrix with material properties: $E_m=$ 2.1 GPa at room temperature (300K), $\nu_m=$ 0.34. The SWCNTs are chosen as the reinforcements and the material properties for the SWCNT are taken from~\cite{zhulei2012} and given in Table \ref{table:cntproperty}. The CNT efficiency parameters $\eta_j$ are determined according to the effective properties of CNTRCs available by matrching the Young's moduli $E_1$ and $E_2$ with the counterparts computed by rule of mixtures. In this study, the efficiency parameters are: $\eta_1=$ 0.149 and $\eta_2=$ 0.934 for the case of $V_{\rm CN}^\ast=$ 0.11; $\eta_1=$ 0.150 and $\eta_2=$ 0.941 for the case of $V_{\rm CN}^\ast=$ 0.14 and $\eta_1=$ 0.149 and $\eta_2=$ 1.381 for the case of $V_{\rm CN}^\ast=$ 0.17. It is assumed that $\eta_2=\eta_3$ for this study.

% CNT material properties: Ref: Composites Part B: 43 (2012), 411-421
\begin{table}[htpb]
\centering
\renewcommand\arraystretch{1.5}
\caption{Temperature dependent material properties for $(10,10)$ SWCNT~\cite{wangshen2012}.}
\begin{tabular}{lrrrrr}
\hline
Temperature & $E_{11}^{\rm CN}$ & $E_{22}^{\rm CN}$ & $G_{12}^{\rm CN}$ & $\alpha_{11}^{\rm CN}$ & $\alpha_{22}^{\rm CN}$ \\
$K$ & (TPa) & (TPa) & (TPa) & $(\times$10$^{-6}$/K$)$ & $(\times$10$^{-6}$/K$)$ \\
\hline
300 & 5.6466 & 7.0800 & 1.9445 & 3.4584 & 5.1682 \\
500 & 5.5308 & 6.9348 & 1.9643 & 4.5361 & 5.0189 \\
700 & 5.4744 & 6.8641 & 1.9644 & 4.6677 & 4.8943 \\
\hline
\end{tabular}
\label{table:cntproperty}
\end{table}


Table \ref{table:mechvalid} presents the convergence of the maximum center deflection with decreasing mesh size for a simply supported square plate subjected to uniformly distributed load with $a/h=$ 20. In this case, the first order shear deformation plate theory (FSDT5) is employed for comparison with the literature~\cite{zhulei2012}. It can be seen that the results from the present formulation are in excellent agreement with the results in the literature and that a 8 $\times$ 8 mesh is found to be adequate to model the full plate for the present analysis. The influence of the CNT volume fraction distribution is also studied. \fref{fig:thruthicknesswdisp} shows the through the thickness transverse displacement for different type of CNT volume fraction distribution. It is seen from \fref{fig:thruthicknesswdisp} that the through the thickness transverse displacements for plates with CNT distributions: UD and FG-X are symmetric with respect to the mid plane, as expected.

% mechanical validation with results from Ref: Composite Structures, v94, 2012, 1450-1460
\begin{table}[htpb]
\centering
\renewcommand\arraystretch{1.5}
\caption{Convergence of maximum center deflection $w_c = -w_o/h \times$10$^{-2}$ with mesh size for a simply supported square plate subjected to uniformly distributed load with $a/h=$ 20.}
\begin{tabular}{lrrr}
\hline
Mesh & \multicolumn{3}{c}{CNT Volume fraction distribution} \\
\cline{2-4}
& UD & FG-V & FG-X \\
\hline
4$\times$4 & 3.0174 & 4.0418 & 2.2710 \\
6$\times$6 & 3.0018 & 4.0209 & 2.2593 \\
8$\times$8 & 2.9993 & 4.0176 & 2.2574 \\
16$\times$116 & 2.9993 & 4.0176 & 2.2574 \\
Ref.~\cite{zhulei2012} & 3.0010 & 4.0250 & 2.2560 \\
\hline
\end{tabular}
\label{table:mechvalid}
\end{table}

% through the thickness w-displacement based on FSDT5
\begin{figure}[htpb]
\newlength\figureheight 
\newlength\figurewidth 
\setlength\figureheight{8cm} 
\setlength\figurewidth{10cm}
\centering
\input{./Figures/Thruthickwdisp.tikz}
\caption{Through the thickness transverse displacement based on FSDT5 for a simply supported square plate with $a/h=$ 50 and $V_{\rm CN}^\ast=$ 0.14.}
\label{fig:thruthicknesswdisp}
\end{figure}

% influence of the volume fraction of the CNT based on FSDT a/b=1, a/h=20
\begin{table}[htpb]
\centering
\renewcommand\arraystretch{1.5}
\caption{Influence of the volume fraction of the CNT, $V_{\rm CN}^\ast$ on the maximum center deflection $w_c = -w_o/h \times$10$^{-2}$ for a simply supported square plate with $a/h=$ 20 based on the first order shear deformation plate theory.}
\begin{tabular}{llrrr}
\hline
& \multicolumn{3}{c}{$V_{\rm CN}^\ast$}\\
\cline{2-4}
& 0.11 & 0.14 & 0.17 \\
\hline
UD & 3.6368 & 2.9993 & 2.3543  \\
FG-V & 4.8866 & 4.0176 & 3.1782  \\
FG-X & 2.7096  & 2.2574 & 1.7438  \\
\hline
\end{tabular}
\label{table:vcntinfluence}
\end{table}
%-------- end of validation
The influence of various plate theories, plate side-to-thickness ratio $a/h$ and CNT volume fraction distribution (viz., UD, FG-V Type, FG-X type) on the maximum center deflection $w_c = -w_o/h$ is shown in Table \ref{table:ahinfluence}. It is seen that decreasing the plate thickness increases the maximum center deflection. For a constant plate thickness, FG-V Type has the maximum center deflection. This can be attributed to the fact that the concentration of the CNT volume fraction distribution at the bottom surface of the plate is minimum. Tables \ref{table:sandwichahinfluence1} - \ref{table:sandwichahinfluence2} presents the influence of plate side-to-thickness $a/h$, core-to-facesheet thickness $hH/hf$ and the volume fraction of the CNT $(V_{\rm CN}^\ast)$ on the deflections and stresses for a sandwich simply supported plate with homogeneous core with a applied sinusoidal load. It is inferred that increasing the core thickness, the non-dimensionalized displaements and stresses decrease, whereas, the displacements and stresses increase with decreasing plate side-to-thickness ratio $a/h$. As before, FG-V Type has the maximum displacements and stresses when compared to the other two CNT distribution, namely, UD and FG-X Type. For a constant plate side-to-thickness ratio, increasing the volume fraction of CNT $(V_{\rm CN}^\ast$, decreases the non-dimensionalized displacements and stresses. This is true irrespective of CNT volume fraction distribution. The through thickness variation of displacements and stresses for a three layer sandwich plate with $a/h=$ 10, $hH/hf=$ 8 and $V_{\rm CN}^\ast=$ 0.28 is shown in \fref{fig:thickdispstress}. In this case, the CNT is assumed to be distributed according to FG-X type. For the loading case considered here, the higher order (HSDT13) and lower-order models (HSDT9 and FSDT5) yield almost similar results. The main difference is that the higher-order models accounts for the slope discontinuity in the in-plane displacements through the thickness, whereas, it is the inclusion of variation up to cubic in the in-plane displacement among the lower-order models. This is evident in the through the thickness in-plane displacements (see \fref{fig:thickdispstress}a).

% influence of the plate thickness
\begin{table}[htpb]
\centering
\renewcommand\arraystretch{1.5}
\caption{Maximum center deflection  for a simply supported square plate subjected to uniformly distributed load with $V_{\rm CN}^\ast=$ 0.17 based on different plate theories.}
\begin{tabular}{llrrr}
\hline
$a/h$ & Element Type & \multicolumn{3}{c}{CNT Volume fraction distribution} \\
\cline{3-5}
& & UD & FG-V & FG-X \\
\hline
\multirow{4}{*}{50} & HSDT11 & 0.7529 & 1.0843 & 0.5155 \\
& HSDT9 & 0.7532 & 1.0849 & 0.5156 \\
& HSDT7 & 0.7480 & 1.0791 & 0.5096 \\
& FSDT5 & 0.7480 & 1.0832 & 0.5151 \\
\cline{2-5}
\multirow{4}{*}{10} & HSDT11 & 2.3746$\times$10$^{-3}$	& 2.9147$\times$10$^{-3}$ &	2.0274$\times$10$^{-3}$ \\
& HSDT9 & 2.3815$\times$10$^{-3}$ & 2.9245$\times$10$^{-3}$ & 2.0285$\times$10$^{-3}$ \\
& HSDT7 & 2.1918$\times$10$^{-3}$ & 2.7065$\times$10$^{-3}$ & 1.8110$\times$10$^{-3}$ \\
& FSDT5 & 2.4022$\times$10$^{-3}$ & 2.8706$\times$10$^{-3}$ & 2.0213$\times$10$^{-3}$ \\
\hline
\end{tabular}
\label{table:ahinfluence}
\end{table}


% influence of plate aspect ratio on the displacements and stresses...
\begin{table}[htpb]
\centering
\renewcommand\arraystretch{1.1}
\caption{Deflections and stresses for a simply supported square sandwich plate with homogeneous core and CNT distributed face-sheets subjected to a sinusoidally distributed load (mechanical load) for two different core thickness $hH/hf=$ 8, 6 and volume fraction of the CNT, $V_{\rm CN}^\ast=$ 0.17.}
\begin{tabular}{llrrrcrrr}
\hline
$hH/hf$ &  & \multicolumn{3}{c}{$S=a/h=$ 10} && \multicolumn{3}{c}{$S=a/h=$ 5} \\
\cline{3-5} \cline{7-9}
& & UD & FG-V & FG-X && UD & FG-V & FG-X \\
\hline
\multirow{5}{*}{8} & $\overline{u}$ & 0.05993 & 0.07868 & 0.05831 && 0.05293 & 0.07846 & 0.05000 \\
&$\overline{w}$ & 0.04104 & 0.05098 & 0.04057 && 0.04469 & 0.05357 & 0.04460 \\
&$\overline{\sigma}_{xx}$ & -0.00654 & -0.00858 & -0.00636 && -0.00577 & -0.00856 & -0.00545 \\
&$\overline{\sigma}_{xy}$ & 0.00543 & 0.00695 & 0.00533 && 0.00525 & 0.00692 & 0.00511 \\
&$\overline{\sigma}_{xz}$ & 0.88089 & 1.14477 & 0.86109 && 0.90434 & 1.25030 & 0.87487 \\
\cline{2-9}
\multirow{5}{*}{6} & $\overline{u}$ & 0.06456 & 0.09358	&	0.06191 &&	0.05388 & 0.09234 & 0.04977 \\
&$\overline{w}$ & 0.04531 & 0.06057 &	0.04453 &&	0.04972 & 0.06289 & 0.04971 \\
&$\overline{\sigma}_{xx}$ & -0.00704 & -0.01021 &	-0.00675 && -0.00588 & -0.01008	& -0.00543 \\
&$\overline{\sigma}_{xy}$ & 0.00593	& 0.00826 & 0.00576 && 0.00565 & 0.00814	 & 0.00546 \\
&$\overline{\sigma}_{xz}$ & 1.16098	& 1.65767 & 1.12147 && 1.12190 & 1.74960	 & 1.07185 \\
\hline
\end{tabular}
\label{table:sandwichahinfluence1}
\end{table}

\begin{table}[htpb]
\centering
\renewcommand\arraystretch{1.1}
\caption{Deflections and stresses for a simply supported square sandwich plate with homogeneous core and CNT distributed face-sheets subjected to a sinusoidally distributed load (mechanical load) for two different core thickness $hH/hf=$ 8, 6 and volume fraction of the CNT, $V_{\rm CN}^\ast=$ 0.28.}
\begin{tabular}{llrrrcrrr}
\hline
$hH/hf$ &  & \multicolumn{3}{c}{$S=a/h=$ 10} && \multicolumn{3}{c}{$S=a/h=$ 5} \\
\cline{3-5} \cline{7-9}
& & UD & FG-V & FG-X && UD & FG-V & FG-X \\
\hline
\multirow{5}{*}{8} & $\overline{u}$ & 0.05178 &	0.07779 & 0.04999	&& 0.04381	& 0.07707 & 0.04118 \\
&$\overline{w}$ &	0.03641 &	0.05048	&	0.03584	&&	0.04071	&	0.05298	&	0.04071 \\
&$\overline{\sigma}_{xx}$ & -0.00664	&	-0.00997	&	-0.00641	&&	-0.00561	&	-0.00988	&	-0.00528	\\
&$\overline{\sigma}_{xy}$ & 0.00476	&	0.00687	&	0.00464 && 0.00459 & 0.00680	&	0.00447 \\
&$\overline{\sigma}_{xz}$ & 1.22873	&	1.82334	&	1.19338 && 1.19037 & 1.92191	&	1.14903	\\
\cline{2-9}
\multirow{5}{*}{6}&$\overline{u}$	& 0.05354 &	0.09216 & 0.05085	&& 0.04230	&	0.09011 & 0.03896	\\
&$\overline{w}$ & 0.03902 &	0.05978 & 0.03816	&& 0.04449 &	0.06196	&	0.04468	\\
&$\overline{\sigma}_{xx}$ & -0.00686 & -0.01181 &	-0.00652	&&	-0.00542	&	-0.01155 & -0.00499	\\
&$\overline{\sigma}_{xy}$ & 0.00502	& 0.00814 &	0.00484 && 0.00480	& 0.00795 & 0.00466	\\
&$\overline{\sigma}_{xz}$ & 1.56428	& 2.63939 &	1.49890 && 1.43423	& 2.70776 & 1.37163	\\
\hline
\end{tabular}
\label{table:sandwichahinfluence2}
\end{table}

% figures...FGM 121 displacement and stress plot through the thickness
\begin{figure}[htpb]
%\newlength\figureheight 
%\newlength\figurewidth 
\setlength\figureheight{8cm} 
\setlength\figurewidth{10cm}
\centering
\subfigure[$\overline{u}$]{\scalebox{0.6}{\input{./Figures/Mudisp.tikz}}}
\subfigure[$\overline{w}$]{\scalebox{0.6}{\input{./Figures/Mwdisp.tikz}}}
\subfigure[$\overline{\sigma}_{xx}$]{\scalebox{0.6}{\input{./Figures/Msxx.tikz}}}
\subfigure[$\overline{\sigma}_{xz}$]{\scalebox{0.6}{\input{./Figures/Msxz.tikz}}}
\caption{Displacements and stresses through the thickness for the square plates with simply supported edges with $a/h=$ 10, $hH/hf=$ 8 and $V_{\rm CN}^\ast=$ 0.28 and the CNT distribution is FG-X.}
\label{fig:thickdispstress}
\end{figure}

==> highOrder_tables.tex <==
% convergence of Q8-HSDT13 element with mesh 
\begin{table}[htpb]
\centering
\renewcommand\arraystretch{1.5}
\caption{Natural frequencies $\Omega = \omega\frac{a^2}{h}\sqrt{\frac{\rho_o}{E_o}}$ for sandwich plates with CNT reinforced facesheets in thermal environment with $a/b=$ 1 and $a/h=$ 20.}
\begin{tabular}{clccc}
\hline
Temperature & Theory & \multicolumn{3}{c}{Frequency parameters} \\
\cline{3-5}
& & $\Omega_1$ & $\Omega_2$ & $\Omega_3$ \\
\hline
\multirow{7}{*}{300}&HSDT13 & 5.0716 & 11.6850 & 13.9750 \\
&HSDT11 & 5.0703 & 11.6760 & 13.9690 \\
%&HSDT11B & 5.0776 & 11.6880 & 14.0950 \\
&HSDT9 & 5.0763 & 11.6790 & 14.0890 \\ 
&HSDT7 & 5.0784 & 11.6980 & 14.0950 \\
&FSDT5 & 5.0735 & 11.6750 & 14.0540 \\
&Ref.~\cite{wangshen2012} & 5.0775 & 11.6798 & 14.0903 \\
\cline{2-5}
\multirow{7}{*}{500}&HSDT13 & 4.8223 & 11.0390 & 13.3560 \\
&HSDT11 & 4.8211 & 11.0300 & 13.3510 \\
%&HSDT11B & 4.8304 & 11.0430	 & 13.5180 \\
&HSDT9 & 4.8292 & 11.0350 & 13.5130 \\
&HSDT7 & 4.8311 & 11.0520 & 13.5170 \\
&FSDT5 & 4.8264 & 11.0300 & 13.4770 \\
&Ref.~\cite{wangshen2012}  & 4.8303 & 11.0352 & 13.5145 \\
\hline
\end{tabular}
\label{vibvalid}
\end{table}

% effect of a/h, volume fraction and type of reinforcement
\begin{table}[htpb]
\centering
\renewcommand\arraystretch{1.5}
\caption{Effect of plate thickness, volume fraction of the nanotubes and type of reinforcement on the fundament frequency parameters $\Omega$ of a simply supported sandwich plate with a homogeneous core. The core-to-facesheet thickness ratio $hH/hf=$ 8 with temperature $T=$ 300$K$.}
\begin{tabular}{clccccccc}
\hline
$a/h$ & Theory & \multicolumn{3}{c}{$V_{\rm CN}=$0.12} && \multicolumn{3}{c}{$V_{\rm CN}=$0.28}\\
\cline{3-5} \cline{7-9}
 &  & UD & V-type & FG && UD & V-type & FG \\
\hline
\multirow{4}{*}{5} &HSDT13 & 4.6057 & 4.3012 & 4.6061 && 4.9850 & 4.3565 & 4.9857 \\
&HSDT11 & 4.5906 & 4.2819 & 4.5913 && 4.9718	 & 4.3064 & 	4.9723 \\
&HSDT9 & 4.6280 & 4.2824 & 4.6542 && 5.0523 & 4.3073 & 5.1032 \\
&FSDT5 & 4.5997 & 4.2794 & 4.6220 && 4.9942 & 4.3030 & 5.0399 \\
\cline{2-9}
\multirow{4}{*}{10} &HSDT13 & 4.9439 & 4.5656 & 4.9634 && 5.4418 & 4.6259 & 5.4849 \\
&HSDT11 & 4.9392 & 4.5584 & 4.9587 && 5.4374 & 4.5857 & 5.4799\\
&HSDT9 & 4.9518 & 4.5586 & 4.9806	 && 5.4661 & 4.5860 & 5.5284\\
&FSDT5 & 4.9428 & 4.5575 & 4.9704 && 5.4468 & 4.5846 & 5.5073\\
\cline{2-9}
\multirow{4}{*}{100} &HSDT13 & 5.0784 & 4.6674 & 5.1083 && 5.6318 & 4.7298 & 5.6999\\
&HSDT11 & 5.0783 & 4.6652 & 5.1081 && 5.6313	& 4.6938 & 5.6985\\
&HSDT9 & 5.0784 & 4.6653 & 5.1083	 && 5.6317	 & 4.6938 & 5.6991\\
&FSDT5 & 5.0783	 & 4.6652 & 5.1082 && 5.6315 & 4.6937 & 5.6988\\
\hline
\end{tabular}
\label{effectofah}
\end{table}

% effect of a/h, volume fraction and type of reinforcement
\begin{table}[htpb]
\centering
\renewcommand\arraystretch{1.5}
\caption{Effect of plate thickness, volume fraction of the nanotubes and type of reinforcement on the fundament frequency parameters $\Omega$ of a simply supported sandwich plate with a homogeneous core. The core-to-facesheet thickness ratio $hH/hf=$ 8 with temperature $T=$ 300$K$.}
\begin{tabular}{clccccccc}
\hline
$hH/hf$ & $V_{\rm CN}$ & \multicolumn{3}{c}{Temperature $T=$ 300$K$} && \multicolumn{3}{c}{Temperature $T=$ 500$K$}\\
\cline{3-5} \cline{7-9}
 &  & UD & V-type & FG && UD & V-type & FG \\
\hline
\multirow{4}{*}{8} & 0.12 & 5.0445 & 4.6419 & 5.0716 && 4.7954 & 4.7391 & 4.8223\\
&0.17 & 5.2404 & 4.6820 & 5.2797 && 4.9913 & 4.4410 & 5.0301\\
&0.28 & 5.5834 & 4.7038 & 5.6447 && 5.3399 & 4.4274 & 5.3992\\
\cline{2-9}
\multirow{4}{*}{6} & 0.12 & 4.8558 & 4.3319 & 4.8992 && 4.6236 & 4.0830 & 4.6662\\
&0.17 & 5.1058 & 4.3844 & 5.6179 && 4.8727 & 4.1240 & 4.9336\\
&0.28 & 5.5339 & 4.4119 & 5.6278 && 5.3055 & 4.1458 & 5.3956\\
\cline{2-9}
\multirow{4}{*}{4} & 0.12 & 4.5716 & 3.8231 & 4.6518 && 4.3650 & 3.5962 & 4.4425\\
&0.17 & 4.9153 & 3.8993 & 5.0277 && 4.7057 & 	3.6559 & 4.8143\\
&0.28 & 5.4803 & 3.9357 & 5.6422 && 5.2713 & 3.6855 & 5.4238\\
\hline
\end{tabular}
\label{effectofcorethick}
\end{table}

==> mechthermalvalid.tex <==
% mechanical and thermal loading validation with 3D results of vel and batra, AIAA J, v40 (7), 2002.

%----------------------------------------------------
% subtables...
%----------------------------------------------------
\begin{table}[htpb]
\caption{The effective material properties are based on the Mori-Tanaka homogenization scheme. The results are based on the HSDT11 element and the gradient index,  $n=$ 1.}
\renewcommand{\arraystretch}{1.25}
\centering
\subtable[Comparison of displacements, stresses for the Al/SiC functionally graded square plate when subjected to a mechanical load. The nondimensionalized physical quantities are: $\overline{u} = 100E_m u/(q_ohS^3), \overline{w} = 100E_m w/(q_ohS^4), (\overline{\sigma}_{xx},\overline{\sigma}_{xy}) = 10(\sigma_{xx}, \sigma_{xy})/(q_oS^3), \overline{\sigma}_{xz}=10\sigma_{xz}/(q_oS)$]{
\centering
\begin{tabular}{clrrrrr}
\hline
$a/h$ & Mesh & \multicolumn{5}{c}{Varaible} \\
\cline{3-7}
& & $\overline{u}$ & $\overline{w}$ & $\overline{\sigma}_{xx}$ & $\overline{\sigma}_{xy}$ & $\overline{\sigma}_{xz}$\\
\hline
\multirow{5}{*}{5} & 4 $\times$ 4 & -2.9305 & 2.5407 & 2.7905 & -1.6545 & 2.2783 \\
& 6 $\times$ 6 & -2.9153 & 2.5512 & 2.7697 & -1.5960 & 2.2985\\
& 8 $\times$ 8 & -2.9129 & 2.5535 & 2.7549 & -1.5783 & 2.3016\\
& 16 $\times$ 16 & -2.9129 & 2.5535 & 2.7549 & -1.5783 & 2.3016\\
& Ref.~\cite{velbatra2002} & -2.9129 & 2.5559 & 2.7562 & -1.5600 & 2.3100\\
\cline{2-7}
\multirow{5}{*}{40} & 4 $\times$ 4 & -2.8972 & 2.1169 & 2.6564 & -1.6470 & 2.3253 \\
& 6 $\times$ 6 & -2.8972 & 2.1148 & 2.5762 & -1.5880 & 2.3287\\
& 8 $\times$ 8 & -2.8967 & 2.1152 & 2.5494 & -1.5704 & 2.3286\\
& 16 $\times$ 16 & -2.8967 & 2.1152 & 2.5494 & -1.5704 & 2.3286\\
& Ref.~\cite{velbatra2002} & -2.8984 & 2.1163 & 2.6093 & -1.5522 & 2.3281\\
\hline
\end{tabular}
%\label{tab:mechvalid}
} \\

% thermal loading...convergence....
\subtable[Comparison of displacements, stresses for the Al/SiC functionally graded square plate when subjected to a thermal load. The nondimensionalized physical quantities are: $\hat{u} = 100u/(h\alpha_m T_o S), \hat{w} = 100w/(h\alpha_mT_oS^2), (\hat{\sigma}_{xx},\hat{\sigma}_{xy},\hat{\sigma}_{xz}) = 10(\sigma_{xx}, \sigma_{xy},\sigma_{xz})/(E_m\alpha_mT_o)$]{
\centering
\begin{tabular}{clrrrrr}
\hline
$a/h$ & Mesh & \multicolumn{5}{c}{Varaible} \\
\cline{3-7}
& & $\hat{u}$ & $\hat{w}$ & $\hat{\sigma}_{xx}$ & $\hat{\sigma}_{xy}$ & $\hat{\sigma}_{xz}$\\
\hline
\multirow{4}{*}{5} & 4 $\times$ 4 & -1.3176 & 4.4726 & -1.2966 & -6.6678 & 2.0430\\
& 6 $\times$ 6 & -1.3232 & 4.4946 & -1.6720 & -7.2500 & 2.3848\\
& 8 $\times$ 8 & -1.3240 & 4.4499 & -1.7445 & -7.1786 & 2.5352\\
& 16 $\times$ 16 & -1.3240 & 4.4499 & -1.7445 & -7.1786 & 2.5352\\
\cline{2-7}
\multirow{4}{*}{40} & 4 $\times$ 4 & -1.2802 & 3.3660 & -1.6954 & -7.2616 & 2.3157\\
& 6 $\times$ 6 & -1.2868 & 3.3795 & -2.0216 & -7.0540 & 2.6674\\
& 8 $\times$ 8 & -1.2878 & 3.3818 & -2.1340 & -6.9832 & 2.8544 \\
& 16 $\times$ 16 & -1.2878 & 3.3818 & -2.1340 & -6.9832 & 2.8544 \\
\hline
\end{tabular}
%\label{tab:thermvalid}
}
\label{fgmvalidation}
\end{table}
